List Message Passing Decoding of Non-binary Low-Density Parity-Check Codes

A decoding algorithm for $q$-ary low-density parity-check codes over the $q$-ary symmetric channel is introduced. The exchanged messages are lists of symbols from $\Fq$. A density evolution analysis for maximum list sizes $1$ and $2$ is developed. Thresholds for selected regular low-density parity-check code ensembles are computed showing gains with respect to a similar algorithm in the literature. Finite-length simulation results confirm the asymptotic analysis.

==> SRLMP ISIT2021 arxiv/tex_files/acron.tex <==
\begin{acronym}
\acro{BEC}{binary erasure channel}
\acro{BSC}{binary symmetric channel}
\acro{BMP}{binary message passing}
\acro{BP}{belief propagation}
\acro{DE}{density evolution}
\acro{LDPC}{low-density parity-check}
\acro{MDPC}{moderate-density parity-check}
\acro{SC-LDPC}{spatially-coupled low-density parity-check}
\acro{lv}{$L$-value}
\acro{llv}{$\bm L$-vector}
\acro{LLR}{low-likelihood ratio}
\acro{QSC}{$q$-ary symmetric channel}
\acro{QEEC}{$q$-ary error and erasure channel}
\acro{SER}{symbol error rate}
\acro{SMP}{symbol message passing}
\acro{VN}{variable node}
\acro{CN}{check node}
\acro{RV}{random variable}
\acro{SC-LDPC}{spatially coupled low-density parity-check}
\end{acronym}


==> SRLMP ISIT2021 arxiv/tex_files/conclusions.tex <==

\section{Conclusions}\label{sec:conclusions}
A decoding algorithm for $q$-ary \ac{LDPC} codes on the \ac{QSC} was introduced and analyzed. We presented a \ac{DE} analysis for maximum list size $1$ and $2$. The \ac{DE} yields iterative decoding thresholds and provides the reliabilities  of the extrinsic channel needed for the \ac{VN} update rule. Our algorithm outperforms competing algorithms with similar complexity.






==> SRLMP ISIT2021 arxiv/tex_files/intro.tex <==
\section{Introduction}\label{sec:Intro}
Non-binary \ac{LDPC} codes have shown an outstanding \EBY{error correction capability,} outperforming their binary counterparts substantially at short block lengths \cite{Davey_nonbin}. Nevertheless, the complexity of the \ac{BP} decoder for these codes  is  high. Various works  reduced the decoding complexity of non-binary \ac{LDPC} codes over \EBY{the} \ac{biAWGN} channel \cite{barnault_fast_2003,declercq_decoding_2007,Zhang_nonbin,Zha_EMS,wany_EMS,declerqNB} and \EBY{the} \ac{QSC} \cite{Luby_verif,matuz_verif,Shokrollahi_qsc,pfister_qsc,smp_lazaro,kurkoski_list}. In  \cite{declercq_decoding_2007}, an extension of the  min-sum algorithm to non-binary fields was presented.
The authors of \cite{Luby_verif} introduced a verification-based decoding algorithm for \ac{LDPC} codes over large alphabet on the \ac{QSC}. Similar approaches were considered in \cite{Shokrollahi_qsc}, \cite{PfisterLMP}.
It has been shown in \cite{Wang_verif} that \ac{LDPC} codes on the \ac{QSC} for large $q$ can approach the Shannon limit. In \cite{kurkoski_list}, the authors introduced a decoding algorithm over the \ac{QSC} (for any $q$) where the exchanged messages are  sets of symbols from $\Fq$ (including the empty set).
%belong to a subset of all possible length $q$ binary vectors. 
The performance of this algorithm improves with the list size, but this comes at the cost of an increasing data flow \EBY{within the decoder, with respect to the case where check and variable nodes exchange only hard decisions (i.e., symbols in $\Fq$)}.


 Inspired by \cite{kurkoski_list}, we propose   a message passing algorithm for $q$-ary \ac{LDPC} codes  over the \ac{QSC}, referred to as \ac{SRLMP}, where the variable and check nodes exchange a set of symbols from $\Fq$ of size at most $\Gamma$. The difference between our algorithm and the one in \cite{kurkoski_list} is the \ac{VN} update rule. In \cite{kurkoski_list}, the channel and the \ac{CN} messages \EBY{are mapped to binary vectors of length $q$. The entry corresponding to the symbol $a \in \Fq$ is one if the message contains the symbol $a$ and it is zero otherwise. These vectors} are summed at the \ac{VN} decoder. Whereas, for \ac{SRLMP} the channel and \ac{CN} messages are converted to log-likelihood vectors at the \acp{VN} by modeling the  extrinsic channel as a \ac{DMC}  whose transition probabilities may be estimated via \ac{DE}. This technique is similar to the \ac{TMP} decoder \cite{benyacoub_tmp} for binary codes, \EBY{and lays its foundation in the \ac{BMP} algorithm originally proposed in \cite{lechner_analysis_2012}}. 

In this work, we describe the \ac{SRLMP} decoder and develop the exact \ac{DE} for $\Gamma\in \{1,2\}$. We provide the iterative decoding thresholds of 
some regular \ac{LDPC} ensembles.



















==> SRLMP ISIT2021 arxiv/tex_files/lmp_DE_1.tex <==
\section{Density Evolution Analysis for \ac{SRLMP} with $\Gamma=1$}\label{sec:DE_lmp_1}
	This section provides a \ac{DE} analysis for \ac{SRLMP} with maximum list size $\Gamma = 1$ for non-binary irregular \ac{LDPC} code ensembles. For $\Gamma =1$, the cardinality of the  message alphabet is $|\cM_1|= q+1$. In the \ac{DE}, the probabilities of \ac{VN} to \ac{CN} and \ac{CN} to \ac{VN}  messages are tracked as iterations progress and we consider the limit as $n \to \infty$. Due to symmetry and under the all-zero codeword assumption, we can partition the message alphabet $\cM_1$ into $3$ disjoint sets $\cI_0, \cI_1, \cI_2$ such that the messages in the same set have the same probability. We have 	
	\begin{align} 
	\cI_0=&\{ \e \} \\
	\cI_1   =& \{ \{0\}\} \label{eq:setslist1} \\
	\cI_2   =& \{ \{a\}: a \in \Fqz\}.
	\end{align}	
Note that $|\cI_0|= |\cI_1| = 1 $, $|\cI_2|=q-1$. Let $\vcm{\cI_k}{\ell}$ be the probability that a \ac{VN} to \ac{CN} message belongs to the set $\cI_k$ at the $\ell$-th iteration, i.e., a \ac{VN} to \ac{CN} message takes the value $a \in \cI_k$ with probability $\vcm{\cI_k}{\ell}/| \cI_k |$. Similarly $\cvm{\cI_k}{\ell}$ is the probability that a \ac{CN} to \ac{VN} message belongs to the set $\cI_k$, where $k \in\{0,1,2\}$.



Initially, we have
	\begin{align}
\vcm{\cI_0}{0}=& 0\\
\vcm{\cI_1}{0}=& 1-\epsilon  \\
\vcm{\cI_2}{0} =& \epsilon.  
\end{align}
At the $\ell$-th iteration, we have
	\begin{align}
	\cvm{\cI_0}{\ell}=& 1- \rho\left(1- \vcm{\cI_0}{\ell-1}\right) \label{eq:s_size1I0} \\
	\begin{split}
	\cvm{\cI_1}{\ell}=&	\frac{1}{q} \Bigg[\rho\left(\vcm{\cI_1}{\ell-1}+\vcm{\cI_2}{\ell-1}\right) \\& + (q-1) \rho\left( \vcm{\cI_1}{\ell-1}-\frac{\vcm{\cI_2}{\ell-1}}{q-1}\right) \Bigg] 
	\end{split} \label{eq:s_size1I1} \\ 
		\begin{split}
	\cvm{\cI_2}{\ell}=&
\frac{q-1}{q} \Bigg[\rho\left(\vcm{\cI_1}{\ell-1}+\vcm{\cI_2}{\ell-1}\right) \\&- \rho\left(\vcm{\cI_1}{\ell-1}-\frac{\vcm{\cI_2}{\ell-1}}{q-1}\right) \Bigg]. \end{split} \label{eq:s_size1I2}
\end{align}
The extrinsic channel  has input alphabet $\inputalphabet=\Fq$, output alphabet $\cZ=\cM_1$ and transition probabilities
\begin{equation}\label{eq:transitionproblist1}
P(z|u)=\begin{cases}
\cvm{\cI_0}{\ell} & \text{if } z=\e \\ 
\cvm{\cI_1}{\ell} & \text{if } z= \{\genfq\} \\
\frac{\cvm{\cI_2}{\ell}}{q-1} & \text{if } z= \{e\} \qquad  e \in \Fq\setminus\{\genfq\}
\end{cases}
\end{equation}
Consider now the \ac{VN} to \ac{CN} messages. We define the random vector $\Fve^{(\ell)}= \left(  \Fl{0}^{(\ell)}, \ldots, \Fl{\alpha^{q-2}}^{(\ell)}, \Fe{\e}^{(\ell)} \right)$, where $\F{\a}^{(\ell)}$ denotes the \ac{RV} associated to the number of  incoming \ac{CN}  messages to a degree $d$ \ac{VN} that take value $\a \in \cM_1$ at the $\ell$-th iteration, and $\fe{\a}^{(\ell)}$  is its realization. The entries of $	\bm{L}\left(\mes{\cn'}{\vn}{\ell}\right)$ in \eqref{eq:LL-vectorlmp} are  
\begin{align}
L_u\left(\mes{\cn'}{\vn}{\ell}\right) = 	\log \left( P(\mes{\cn'}{\vn}{\ell}|u) \right)
\end{align}
	where $\mes{\cn'}{\vn}{\ell} \in \cM_1, u\in \Fq$ and $P(z|u)$ is given in \eqref{eq:transitionproblist1} $\forall z \in \cM_1$.
%\begin{align}
Hence, the elements $\aggc{u}{\ell}$ of the  extrinsic \acl{llv}  in \eqref{eq:LL-vectorlmp} are 
\begin{align}
\aggc{\genfq}{\ell} =&
\D^{(\ell)}_1 \fl{\genfq}^{(\ell)} + \D_{\tch} \delta_{\genfq y} \EBY{+ K_1}
\end{align} 
\EBY{where 
	\begin{align} 
	\begin{split}\label{eq:Klist1}
		K_1=&\log(\epsilon/(q-1))+ \fe{\e}^{(\ell)} \log(\cvm{\cI_0}{\ell})\\&+(d-1-\fe{\e}^{(\ell)}) \log(\cvm{\cI_2}{\ell} /(q-1) )
	\end{split}\\
\D_{\tch} =& \log(1-\epsilon)-\log(\epsilon/(q-1))  \label{eq:Dch}\\
\D^{(\ell)}_1=& \log(\cvm{\cI_1}{\ell})- \log(\cvm{\cI_2}{\ell}/(q-1)) \label{eq:D1}
\end{align}
and $ \delta_{ij} $ is the Kronecker delta function. Note that $K_1$ in \eqref{eq:Klist1} is independent of $\genfq$. Thus, it can be ignored when computing the extrinsic \acl{llv}.}


We obtain
\begin{align}
\begin{split}
 \vcm{\cI_0}{\ell} =& \sum\limits_{d} \lambda_d \sum_{y\in \Fq } \Pr\{Y=y\}  \sum_{\fve^{(\ell)} } \Pr\{\Fve^{(\ell)}=\fve^{(\ell)} \} \times \\ & \left[1 - \sum\limits_{a \in \Fq}\prod\limits_{\genfq \in \Fqa}\I (\aggc{a}{\ell} > \aggc{\genfq}{\ell} + \Delta^{(\ell)}) \right]
 \end{split}\\
 \begin{split}
 \vcm{\cI_1}{\ell} =& \sum\limits_{d} \lambda_d \sum_{y \in \Fq } \Pr\{Y=y\}  \sum_{\fve^{(\ell)} } \Pr\{\Fve^{(\ell)}=\fv^{(\ell)} \} \times  \\ & \prod\limits_{\genfq \in \Fqz} \I (\aggc{0}{\ell} > \aggc{\genfq}{\ell} + \Delta^{(\ell)})
 \end{split} \\ 
  \vcm{\cI_2}{\ell} =& 1-\vcm{\cI_0}{\ell}- \vcm{\cI_1}{\ell}.
    \end{align}
where   $\I(\cA)$ is an indicator function and  the inner sum is over all length $q+1$ non-negative integer vectors $\bm{f}^{(\ell)}$ whose entries  sum to $d-1$ and
\begin{align}
\Pr\{\bm{F}^{(\ell)}=\bm{f}^{(\ell)}\} =& \binom{d-1}{\fl{0}^{(\ell)},\ldots,\fe{\e}^{(\ell)}}  \prod\limits_{k=0}^{2}\left(\frac{\cvm{\cI_k}{\ell}}{| \cI_k|}\right)^{f_{\cI_k}^{(\ell)}}    \\
f_{\cI_k}^{(\ell)}=&\sum\limits_{a \in \cI_k}\f{a}^{(\ell)} \quad \forall k \in \{0,1,2\}.
\end{align}
The iterative decoding threshold $\proberror^\star$ is the maximum \EBY{ \ac{QSC}} error probability such that $ \vcm{\cI_1}{\ell} \to 1$ as $\ell \to \infty$.


==> SRLMP ISIT2021 arxiv/tex_files/lmp_DE_2.tex <==
\section{Density Evolution Analysis for \ac{SRLMP} with $\Gamma=2$}\label{sec:DE_lmp_2}
This section gives a \ac{DE} analysis for \ac{SRLMP} with maximum list size $\Gamma = 2$.  For $\Gamma=2$, the cardinality of the message alphabet is $|\cM_2|= 1+ q+\binom{q}{2}$.  Due to symmetry and under the all-zero codeword assumption, we can partition the message alphabet $\cM_2$ into $5$ disjoint sets $\cI_0, \cI_1, \cI_2, \cI_3, \cI_4$ such that the messages in the same set have the same probability. We have $\cI_0, \cI_1, \cI_2$ as defined in \eqref{eq:setslist1} and	
\begin{align}
	    \cI_3=& \left\{ \{0,a\}: a \in  \Fqz \right\}\\
	    \cI_4=& \left\{ \{a,e\}: a,e \in  \Fqz \text{ and } a \neq e \right\}
	\end{align}
Note that $|\cI_0|= |\cI_1| = 1 $, $|\cI_2|=|\cI_3|=q-1$ and $|\cI_4|= \binom{q-1}{2}$.	Let $\vcm{\cI_k}{\ell}$ be the probability that a \ac{VN} to \ac{CN} message belongs to the set $\cI_k$ at the $\ell$-th iteration. Similarly $\cvm{\cI_k}{\ell}$ is the probability that a \ac{CN} to \ac{VN} message belongs to the set $\cI_k$, where $k \in\{0,1,2,3,4\}$.
	
	Initially, we have
	\begin{align}
	&\vcm{\cI_1}{0}= 1-\epsilon \\
	&\vcm{\cI_2}{0}= \epsilon\\
	&\vcm{\cI_0}{0} = \vcm{\cI_3}{0}=\vcm{\cI_4}{0}=0.  
	\end{align}
	For the \ac{CN} to \ac{VN} messages,  $\cvm{\cI_1}{\ell}$, $\cvm{\cI_2}{\ell}$, $\cvm{\cI_3}{\ell}$, $\cvm{\cI_4}{\ell}$ are given in \eqref{eq:s_size1I1}, \eqref{eq:s_size1I2},  \eqref{eq:si2} and \eqref{eq:si3}, respectively and 
	\begin{align}
	\cvm{\cI_0}{\ell}=1-\cvm{\cI_1}{\ell}-\cvm{\cI_2}{\ell}-\cvm{\cI_3}{\ell}-\cvm{\cI_4}{\ell}.
 \end{align}
	\begin{figure*}
	%	\vspace{-3mm}
	\begin{align}
	\begin{split}\label{eq:si2}
\cvm{\cI_3}{\ell}=&\frac{q-1}{q} \Bigg[-2\rho \left(\vcm{\cI_1}{\ell-1}+\vcm{\cI_2}{\ell-1}\right)+2\rho \left( \vcm{\cI_1}{\ell-1}+\vcm{\cI_2}{\ell-1}+\frac{\vcm{\cI_3}{\ell-1}}{q-1}+\frac{\vcm{\cI_4}{\ell-1}}{q-1}\right) 
	\\ & +(q-2) \rho\left( \vcm{\cI_1}{\ell-1}-\frac{\vcm{\cI_2}{\ell-1}}{q-1}+\frac{\vcm{\cI_3}{\ell-1}}{q-1}-\frac{2\vcm{\cI_4}{\ell-1}}{(q-1)(q-2)}\right) -(q-2)\rho\left(\vcm{\cI_1}{\ell-1}-\frac{\vcm{\cI_2}{\ell-1} }{q-1}\right)\Bigg]
\end{split}\\
\begin{split}\label{eq:si3}
\cvm{\cI_4}{\ell}=&\frac{(q-1)(q-2)}{q} \Bigg[\rho \left( \vcm{\cI_1}{\ell-1}+\vcm{\cI_2}{\ell-1}+\frac{\vcm{\cI_3}{\ell-1}}{q-1}+\frac{\vcm{\cI_4}{\ell-1}}{q-1}\right) -\rho\left(\vcm{\cI_1}{\ell-1}+\vcm{\cI_2}{\ell-1}\right) \\ & -\rho\left( \vcm{\cI_1}{\ell-1}-\frac{\vcm{\cI_2}{\ell-1}}{q-1}+\frac{\vcm{\cI_3}{\ell-1}}{q-1}-\frac{2\vcm{\cI_4}{\ell-1}}{(q-1)(q-2)}\right) +\rho\left(\vcm{\cI_1}{\ell-1}-\frac{\vcm{\cI_2}{\ell-1}}{q-1}\right)\Bigg] 
\end{split}
\end{align}
	\vspace{-2mm}
\hrule
\end{figure*}
In this case, the extrinsic channel  has input alphabet $\inputalphabet=\Fq$, output alphabet $\cZ=\cM_2$ and transition probabilities
		\begin{equation}\label{eq:transitionproblist}
	P(z|u)=\begin{cases}
	\cvm{\cI_0}{\ell} & \text{if } z= \{\genfq\} \\
	\frac{\cvm{\cI_1}{\ell}}{|\cI_1|} & \text{if } z= \{e\} \qquad  e \in \Fq\setminus\{\genfq\}\\
	\frac{\cvm{\cI_2}{\ell}}{|\cI_2|} & \text{if } z= \{\genfq,e\}\quad  e \in \Fq\setminus\{\genfq\}\\
	\frac{\cvm{\cI_3}{\ell}}{|\cI_3|} & \text{if } z= \{a,e\} \quad  a,e \in \Fq\setminus\{\genfq\}\\
	\cvm{\cI_4}{\ell} & \text{if } z=\e.
	\end{cases}
	\end{equation}
	Consider now the \ac{VN} to \ac{CN} messages. We extend the random vector $\Fv^{(\ell)}$ to 
	\[
	\Fvl^{(\ell)}= \left(  \Fl{0}^{(\ell)}, \ldots, \Fl{\alpha^{q-2}}^{(\ell)}, \Fl{0,1}^{(\ell)} , \ldots, \Fl{\alpha^{q-3},\alpha^{q-2}}^{(\ell)} ,\Fe{\e}^{(\ell)} \right),
	\]
	where $\F{\a}^{(\ell)}$ denotes the \ac{RV} associated to the number of  incoming \ac{CN}  messages to a degree $d$ \ac{VN} that take value $\a \in \cM_2$ at the $\ell$-th iteration. The entries of $	\bm{L}\left(\mes{\cn'}{\vn}{\ell}\right)$ in \eqref{eq:LL-vectorlmp} are given  by  
	\begin{align}
	L_u\left(\mes{\cn'}{\vn}{\ell}\right) = 	\log \left( P(\mes{\cn'}{\vn}{\ell}|u) \right)
	\end{align}
	where $\mes{\cn'}{\vn}{\ell} \in \cM_2, u\in \Fq$ and $P(z|u)$ is given in \eqref{eq:transitionproblist} $\forall z \in \cM_2$.
	%\begin{align}
		Hence, the entries $\aggc{u}{\ell}$ of the aggregated extrinsic \acl{llv}  in \eqref{eq:LL-vectorlmp} are related to $\f{\genfq}^{(\ell)}$ and the channel observation $y$ by
\begin{align}
\aggc{\genfq}{\ell} &=
\D_1^{(\ell)} \fl{\genfq}^{(\ell)}+  \D_2^{(\ell)} \sum\limits_{a \in \Fq \setminus \{\genfq\}}\fl{\genfq,a}^{(\ell)}+ \D_{\tch} \delta_{\genfq y} \EBY{+ K_2}
\end{align} 
where $\D_{\tch}$ and $\D^{(\ell)}_1$ are given in \eqref{eq:Dch} and \eqref{eq:D1} and we have
\begin{align}
\D_2^{(\ell)}=&\log\left(\cvm{\cI_3}{\ell}/|\cI_3|\right) - \log\left(\cvm{\cI_4}{\ell}/|\cI_4|\right)\\
\begin{split} \label{eq:Klist2}
K_2=& \log(\epsilon/(q-1)) + \sum\limits_{a \in \Fq} \fl{a}^{(\ell)} \log\left(\cvm{\cI_2}{\ell}/|\cI_2|\right) \\&+ \sum\limits_{a,e \in \Fq} \fl{a,e}^{(\ell)} \log\left(\cvm{\cI_4}{\ell}/|\cI_4| \right)+ \fe{\e}^{(\ell)} \log(\cvm{\cI_0}{\ell}).
\end{split}
\end{align} 
Note that $K_2$ in \eqref{eq:Klist2} can be ignored in the \ac{VN} update rule since  it is independent of $\genfq$.


We obtain
\begin{align}
		\begin{split}
	\vcm{\cI_1}{\ell} =& \sum\limits_{d} \lambda_d \sum\limits_{y\in \Fq}\Pr\{Y=y\}\sum\limits_{\bm{f}^{(\ell)}}\Pr\{\bm{F}^{(\ell)}=\bm{f}^{(\ell)}\} \times \\& \prod\limits_{\genfq\in \Fqz}
	\I (\aggc{0}{\ell} > \aggc{\genfq}{\ell} + \Delta^{(\ell)})
		\end{split}\\
		\begin{split}
		\vcm{\cI_2}{\ell}=& \sum\limits_{d} \lambda_d\sum\limits_{a\in \Fqz} \sum\limits_{y\in \Fq}\Pr\{Y=y\}\sum\limits_{\bm{f}^{(\ell)}}\Pr\{\bm{F}^{(\ell)}=\bm{f}^{(\ell)}\}\\ &\prod\limits_{\genfq\in \Fqa}	\I (\aggc{a}{\ell} > \aggc{\genfq}{\ell} + \Delta^{(\ell)})
		\end{split} \\ 
	\begin{split}
	\vcm{\cI_3}{\ell}=& \sum\limits_{d} \lambda_d  \sum\limits_{y\in \Fq}\Pr\{Y=y\}  \sum\limits_{\bm{f}^{(\ell)}}\Pr\{\bm{F}^{(\ell)}=\bm{f}^{(\ell)}\}  \times    \\&   \sum\limits_{a\in \Fqz}   \I\left(| \aggc{0}{\ell}-\aggc{a}{\ell}| \leq \Delta ^{(\ell)} \right) \times  \\ &\prod\limits_{\genfq\in \Fq\setminus\{0,a\}}\I\left(\aggc{a}{\ell}>\aggc{\genfq}{\ell} + \Delta^{(\ell)}\right)  \I\left(\aggc{0}{\ell}> \aggc{\genfq}{\ell}+ \Delta^{(\ell)}\right)
		\end{split} \\
\begin{split}
		\vcm{\cI_4}{\ell}=& \sum\limits_{d} \lambda_d  \sum\limits_{y\in \Fq}\Pr\{Y=y\}  \sum\limits_{\bm{f}^{(\ell)}}\Pr\{\bm{F}^{(\ell)}=\bm{f}^{(\ell)}\} \times 
	 \\ & 	\sum\limits_{a,e\in \Fq \setminus \{0\},a\neq e} \mathbb{I}\left(| \aggc{a}{\ell}-\aggc{e}{\ell}| \leq \Delta^{(\ell)}\right)  \times \\ & \prod\limits_{u\in \Fq\setminus\{a,e\}}\mathbb{I}\left(\aggc{a}{\ell}> \aggc{u}{\ell}+ \Delta ^{(\ell)} \right)  \I\left(\aggc{e}{\ell}> \aggc{u}{\ell} + \Delta^{(\ell)} \right) 
\end{split} \\
	\vcm{\cI_0}{\ell}=&1-	\vcm{\cI_1}{\ell}-	\vcm{\cI_2}{\ell}-	\vcm{\cI_3}{\ell}-	\vcm{\cI_4}{\ell}
	\end{align}
	where the inner sum is over all length $|\cM_2|$ non-negative integer vectors $\bm{f}^{(\ell)}$ whose entries  sum to $d-1$
\begin{align}
 \Pr\{\bm{F}^{(\ell)}=\bm{f}^{(\ell)}\} =& \binom{d-1}{\fl{0}^{(\ell)},\ldots,\fe{\e}^{(\ell)}}  \prod\limits_{k=0}^{4}\left(\frac{\cvm{\cI_k}{\ell}}{| \cI_k|}\right)^{f_{\cI_k}^{(\ell)}}    \\
  f_{\cI_k}^{(\ell)}=&\sum\limits_{a \in \cI_k}\f{a}^{(\ell)} \quad \forall k \in \{0,\ldots,4\}.
\end{align}
	The iterative decoding threshold $\proberror^\star$ is defined as the  maximum channel error probability such that $ 	\vcm{\cI_1}{\ell} \to 1$ as $\ell \to \infty$.


==> SRLMP ISIT2021 arxiv/tex_files/lmp_description.tex <==
\section{\ac{SRLMP} Decoding}\label{sec:lmp_description}
This section  introduces an extension of the \ac{SMP} algorithm \cite{smp_lazaro} for transmission over a \ac{QSC}. An exchanged message between a check and a variable node is a list of symbols from $\Fq$ of size between $0$ (empty set) and  $\Gamma$, i.e., the message alphabet is $\cM_\Gamma$ which  contains all possible sets of symbols in $\Fq$ of size less \EBY{than} or equal \EBY{to} $\Gamma$ (including the empty set). The cardinality of the message alphabet is $|\cM_\Gamma| = \sum\limits_{i=0}^{\Gamma} \binom{q}{i}$. 
%\Com{The empty set represents an erasure to denote complete uncertainty about the  respective symbol value.}
%\[|\cM_\Gamma| = \sum\limits_{i=0}^{\Gamma} \binom{q}{i}\].

\begin{enumerate}[label=\roman*.]
	\item \textbf{Initialization.}
	
		Each \ac{VN} sends its channel observation $y$ to its neighboring \acp{CN}: 
		\begin{equation}
	\mes{\vn}{\cn}{0}=y.
\end{equation}
\smallskip
	\item \textbf{Check to variable update}
	
	  \EBY{Consider a \ac{CN} $\cn$ and a \ac{VN} $\vn$ connected to it. If  all of the incoming messages to $\cn$ from the other neighboring \acp{VN} are not empty, $\cn$} computes the set of all symbols that satisfy the parity check equation given the received \ac{VN} messages. Formally, \EBY{it} computes
		\begin{equation} \label{eq:CNlist}
		    \cU_{\vn,\cn}^{(\ell)}=- h_{\vn,\cn}^{-1}\sum\limits_{\vn' \in \cN (\cn) \setminus \vn} h_{\vn',\cn} \mes{\vn'}{\cn}{\ell-1}.
		\end{equation}
		 The multiplication in \eqref{eq:CNlist} is performed element-wise over $\Fq$ and the sum is over sets of symbols. The sum over two sets $\cA$ and $\cB$ is defined as \EBY{the Minkowski sum, i.e.,}
		\begin{equation}
		    \cA + \cB = \{a+b: a \in \cA, b \in \cB \}.
		\end{equation}
		If the size of $\cU_{\vn,\cn}^{(\ell)}$ is larger than $\Gamma$ or  $\cn$ receives at least one empty set from its neighboring \acp{VN}, then $\cn$ sends an empty set to $\vn$, otherwise it sends the set $\cU_{\vn,\cn}^{(\ell)}$. Formally, we write
		\begin{equation} 
		      \mes{\cn}{\vn}{\ell} = \begin{cases}
		     \cU_{\vn,\cn}^{(\ell)}  & \begin{aligned} & \text{if }\mes{\vn'}{\cn}{\ell-1} \neq \e  \, \, \forall \vn' \in \cN(\cn)\setminus \vn  \\ & \text{ and }  |\cU_{\vn,\cn}^{(\ell)}| \leq \Gamma  \end{aligned} \\ 
		    \e & \text{otherwise}.
		      \end{cases}
		\end{equation}
	\smallskip
		\item  \textbf{Variable to check update}
		
	\EBY{First, each \ac{VN}}  computes 
	\begin{equation}
		\begin{aligned} \label{eq:LL-vectorlmp}
		\aggv{\ell}&=\left[\aggc{0}{\ell},\aggc{1}{\ell},\ldots,\aggc{\alpha^{q-2}}{\ell} \right]\\ 
		&= \bm{L}\left(y\right) + \sum_{\cn' \in \neigh{\vn} \setminus \cn}  \bm{L}\left(\mes{\cn'}{\vn}{\ell}\right). 
	\end{aligned}
\end{equation}
Then, the outgoing \ac{VN} message is obtained by applying Algorithm \ref{alg:vnupdate}.
\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\State Initialize the set $\cT= \emptyset$
		\State Find one symbol $a \in \Fq$ with $\aggc{a}{\ell}= \max\limits_{u \in \Fq \setminus \cT} \aggc{u}{\ell}$ \label{state:addVN}
		\State Update the set  $\cT = \cT \cup \{a\}$
		\If{$\aggc{e}{\ell} > \aggc{u}{\ell} + \Delta^{(\ell)} \, \, \forall e \in \cT $ and $\forall u \in \Fq \setminus \cT$}
		\State $  \mes{\vn}{\cn}{\ell} =\cT$
		\Else 
		\If{$|\cT|< \Gamma$}
		\State return to \ref{state:addVN}
		\Else 
		
		     $ \quad  \mes{\vn}{\cn}{\ell} =\e$
		\EndIf
		\EndIf
	\end{algorithmic}
	\caption{\ac{VN} Update Rule.}
	\label{alg:vnupdate}
\end{algorithm}
For $\Gamma=1$, Algorithm \ref{alg:vnupdate} simplifies to 
\begin{align}
 \mes{\vn}{\cn}{\ell} = \begin{cases}
 \{a\} & \begin{aligned} & \text{if } \exists a \in \Fq: \aggc{a}{\ell} > \aggc{u}{\ell} + \Delta^{(\ell)} \\&  \forall u \in \Fq \setminus \{a\}  \end{aligned} \\
 \e & \text{otherwise}
\end{cases}
\end{align}
and for $\Gamma=2$ 
\begin{align}
\mes{\vn}{\cn}{\ell} = \begin{cases}
\{a\} & \begin{aligned} & \text{if } \exists a \in \Fq: \aggc{a}{\ell} > \aggc{u}{\ell} + \Delta^{(\ell)} \\&  \forall u \in \Fq \setminus \{a\} \end{aligned} \\
\{a,e\} & \begin{aligned} &\text{if } \exists a,e \in \Fq: |\aggc{a}{\ell}  - \aggc{e}{\ell} | \leq \Delta^{(\ell)} \\& \text{and } \aggc{a}{\ell}, \aggc{e}{\ell} > \aggc{u}{\ell} +\Delta^{(\ell)} \\& \forall u \in \Fq \setminus \{a,e\} \end{aligned}\\
\e & \text{otherwise}.
\end{cases}
\end{align}
	 In \eqref{eq:LL-vectorlmp}, the \acl{llv} $\bm{L}(y)$ corresponding to the channel observation is obtained from  \eqref{eq:llvector2} using the transition probabilities of the \ac{QSC} communication channel given in \eqref{eq:QSC_trans_prob}. Further, we model each \ac{CN} to \ac{VN} message as an observation of the symbol $X$ (associated to $\vn$) at the output of an \emph{extrinsic channel}  with input alphabet $\inputalphabet= \Fq$ and output alphabet $\cZ= \cM_\Gamma$. The transition probabilities of the extrinsic channel can be estimated via \ac{DE} and are  used to compute the \aclp{llv} of the \ac{CN} messages as shown in  \eqref{eq:llvector} and \eqref{eq:llvector2}. The parameters $\Delta^{(\ell)}$ are chosen to maximize the iterative decoding threshold and can be chosen for each iteration individually.
 \smallskip
	\item \textbf{Final decision.} 
	
		Each variable node computes 
		\begin{align}
		\aggappvl{\ell}&=\left[\aggappl{0}{\ell},\aggappl{1}{\ell},\ldots,\aggappl{\alpha^{q-2}}{\ell} \right]\\ 
		&= \bm{L}\left(y\right) + \sum_{\cn' \in \neigh{\vn} } \bm{L}\left(\mes{\cn'}{\vn}{\ell}\right) .
	\end{align}
	\begin{align}\label{eq:finaldecision}
	\hat{x}^{(\ell)} = \argmax{\genfq \in \Fq}  \aggappl{\genfq}{\ell}.
\end{align}
In \eqref{eq:finaldecision}, if multiple maximizing arguments exist  we choose one of them uniformly at random.
	\end{enumerate}
Note that for $\Gamma=1$, the \ac{SRLMP} is similar to the \ac{SMP} \cite{smp_lazaro} but \ac{SRLMP} includes an additional empty set.

==> SRLMP ISIT2021 arxiv/tex_files/notation.tex <==
\newtheorem{remark}{Remark}



\newcommand{\dv}{\mathsf{d_{v}}}
\newcommand{\dc}{\mathsf{d_{c}}}
\newcommand{\dvj}{\mathsf{d_{v_{j}}}}
\newcommand{\dci}{\mathsf{d_{c_{i}}}}
\newcommand{\dvmax}{\mathsf{d_{v}^{\text{max}}}}
\newcommand{\dcmax}{\mathsf{d_{c}^{\text{max}}}}

\newcommand{\inputalphabet}{\mathcal{X}}
\newcommand{\inputrv}{X}
\newcommand{\inputrvreal}{x}
\newcommand{\outputalphabet}{\mathcal{Y}} 
\newcommand{\outputrv}{Y}
\newcommand{\outputrvreal}{y}

\newcommand{\messagealphabet}{\mathcal{M}}

\newcommand{\proberror}{\epsilon}
\newcommand{\proberasure}{\gamma}
\newcommand{\ns}{{\eta}}

\newcommand{\normterm}{\delta}
	
\newcommand{\Rc}{R}

\newcommand{\Cirreg}{\mathscr{C}_{q}^{\lambda,\rho}}
\newcommand{\ensC}[3]{\mathscr C_{ #1, #2}^{#3}}
\newcommand{\ensSC}[3]{\bm{B}_{ #1, #2}^{#3}}
\newcommand{\vn}{\mathtt{v}}%variable node

\newcommand{\cn}{\mathtt{c}}%check node

\newcommand{\cm}{r}%channel message


\newcommand{\cN}{\mathcal{N}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cI}{\mathcal{I}}


\newcommand{\vcm}[2]{p_{#1}^{(#2)}}%pr  of var to check node message
\newcommand{\cvm}[2]{s_{#1}^{(#2)}}
\newcommand{\cvmvec}[1]{\bm{s}^{(#1)}}
\newcommand{\vcmvec}[1]{\bm{p}^{(#1)}}
\newcommand{\vcmvecFP}{\bm{p}^{\star}}
\newcommand{\cvmvecFP}{\bm{s}^{\star}}


\newcommand{\vcmirreg}[2]{\bar{p}_{#1}^{(#2)}}%pr  of var to check node message
\newcommand{\cvmirreg}[2]{\bar{s}_{#1}^{(#2)}}

\newcommand{\vapp}[1]{P_{\tapp}^{(#1)}} %decision variable node
\newcommand{\vcmlong}[2]{P_{\outputrv|\inputrv}^{(#2)}(#1|0) }%pr  of var to check node message
\newcommand{\cvmlong}[2]{P_{S|\inputrv}^{(#2)}(#1|0) }%pr  of var to check node message
\newcommand{\vcmFP}[1]{p_{#1}^{\star}}
\newcommand{\cvmFP}[1]{s_{#1}^{\star}}


\newcommand{\vect}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\neigh}[1]{\mathcal{N} ( #1) }



\newcommand{\mes}[3]{m_{ #1 \rightarrow #2 }^{(#3)}}
\newcommand{\Mes}[3]{M_{ #1 \rightarrow #2 }^{(#3)}}

\newcommand{\mesch}[1]{m_{ #1 }}

\newcommand{\minr}{m_{ \text{in}}}
\newcommand{\minrv}[1]{M^{(#1)}_{ \text{in}}}

\newcommand{\vecgen}{u}

\newcommand{\comp}{{\Psi}}

\newcommand{\Fq}{\mathbb{F}_q}
\newcommand{\Fqz}{\mathbb{F}_q \setminus \{0\}}
\newcommand{\Fqa}{\mathbb{F}_q \setminus \{a\}}

\renewcommand{\argmax}[1]{\underset{#1}{\mathrm{arg \, max}}\,}

\newcommand{\mesvec}[2]{\bm{z}_{#1 \rightarrow #2}}

\ifdef{\l}
{\renewcommand{\l}[1]{L_{ #1}} }
{\newcommand{\l}[1]{L_{ #1}}}

\newcommand{\lv}{\bm{L}}

\newcommand{\lin}[1]{\sigma^{(#1)}}
\newcommand{\linv}[1]{\bm{\sigma}^{(#1)}}

\newcommand{\linapp}[1]{l^{(#1)}}
\newcommand{\linappv}[1]{\bm{l}^{(#1)}}

\newcommand{\papp}[1]{P_{\text{app}}^{(#1)}}

\newcommand{\genfq}{u}



\newcommand{\linvi}[3]{\bm{l}_{ #1 \rightarrow #2}^{(#3)} }
\newcommand{\lini}[3]{l_{ #1 \rightarrow #2}^{(#3)} }

\newcommand{\lch}[1]{l_{\text{ch}, #1}}
\newcommand{\lchv}{\bm{l}_{\text{ch}}}

\newcommand{\F}[1]{F_{#1}}
\newcommand{\f}[1]{f_{#1}}
\newcommand{\tF}[1]{\tilde{F}_{#1}}
\newcommand{\tf}[1]{\tilde{f}_{#1}}

\newcommand{\Fv}{\bm{F}}
\newcommand{\fv}{\bm{f}}
\newcommand{\tFv}{\bm{\tilde{F}}}
\newcommand{\tfv}{\bm{\tilde{f}}}

\newcommand{\fve}{\bm{f}}
\newcommand{\Fe}[1]{F_{#1}}
\newcommand{\fe}[1]{f_{#1}}
\newcommand{\tFe}[1]{\tilde{F}_{#1}}
\newcommand{\tfe}[1]{\tilde{f}_{#1}}
\newcommand{\Fve}{\bm{F}}
\newcommand{\tFve}{\bm{\tilde{F}}}
\newcommand{\tfve}{\bm{\tilde{f}}}


\newcommand{\fvl}{\bm{f}}
\newcommand{\Fl}[1]{F_{\{#1\}}}
\newcommand{\fl}[1]{f_{\{#1\}}}
\newcommand{\Flp}[2]{F_{\{#1\},#2}} %proto
\newcommand{\flp}[2]{f_{\{#1\},#2}}
\newcommand{\tflp}[2]{\tilde{f}_{\{#1\},#2}}
\newcommand{\tFl}[1]{\tilde{F}_{\{#1\}}}
\newcommand{\tfl}[1]{\tilde{f}_{\{#1\}}}
\newcommand{\Fvl}{\bm{F}}
\newcommand{\tFvl}{\bm{\tilde{F}}}
\newcommand{\tfvl}{\bm{\tilde{f}}}



\newcommand{\Dch}{D_{\text{ch}}}
\newcommand{\Dex}{D_{\text{ex}}}

\newcommand{\I}{\mathbb{I}}
\newcommand{\argI}{\mathcal B}

\renewcommand{\a}{a}
\renewcommand{\b}{y}
\renewcommand{\u}{u}

\newcommand{\nbit}{l}
\newcommand{\hw}{\mathrm d_{\mathrm{H}}}

\newcommand{\cellfreq}{z}

\newcommand{\agg}{L_{\mathsf{ex}}}
\newcommand{\aggc}[2]{L^{(#2)}_{\mathsf{ex},#1}}
\newcommand{\aggv}[1] {\bm{L}^{(#1)}_{\mathsf{ex}}}
\newcommand{\lmaxim}[1]{\mathcal{L^{(#1)}_{\mathsf{ex}}}}

\newcommand{\aggappvl}[1]{{\bm{L}^{(#1)}_{\mathsf{app}}}} %app l-th iteration
\newcommand{\aggappl}[2]{{L^{(#2)}_{\mathsf{app},#1}}}
\newcommand{\lmaximapp}[1]{\mathcal{L^{(#1)}_{\mathsf{app}}}}

\newcommand{\Mcdf}{P}
\newcommand{\Mpdf}{\rho}

\newcommand{\Xa}{A}
\newcommand{\xa}{a}
\newcommand{\Ya}{B}
\newcommand{\ya}{b}

\newcommand{\binv}[1]{\bm{#1}_{\mathrm{b}}}
\newcommand{\mapbin}[1]{{_b}\left(#1\right) }

\ifdef{\H}
{\renewcommand{\H}{\mathsf{U}}}
{\newcommand{\H}{\mathsf{U}}}

\ifdef{\D}
{\renewcommand{\D}{\mathsf{D}}}
{\newcommand{\D}{\mathsf{D}}}

\newcommand{\W}{\mathsf{W}}

\newcommand{\nmax}[1] { \underset{#1}{\#\mathrm{max} }} %
\newcommand{\nel}[1]{{\mu}_{#1} } %
\newcommand{\nmaxr}{\kappa}
\newcommand{\nmaxrmax}{\kappa_{\mathrm{max}}}


\newcommand{\accvote}[1]{{t_{#1}}}
	
\newcommand{\az}{\accvote{0}}
\newcommand{\ao}{\accvote{1}}


\newcommand{\fmax}{f_{\text{max}}}


\newcommand{\tapp}{\text{app}}
\newcommand{\tmax}{\text{max}}
\newcommand{\tch}{\text{ch}}

\newcommand{\lmp}{LMP }
\newcommand{\e}{\mathcal{E}} % erasure 

==> SRLMP ISIT2021 arxiv/tex_files/packages.tex <==
\usepackage{amsmath,amsthm,amssymb,graphicx,cite,bm}
\usepackage{epsfig,amsfonts}
\usepackage{graphicx}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\usepackage[nolist]{acronym}
\usepackage{psfrag}
\usepackage{perso}
\usepackage{makecell}
\usepackage{enumitem}
\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother
%
%\bibliographystyle{IEEEtran}
%\setlength{\arraycolsep}{0.07 cm}
%
%\IEEEoverridecommandlockouts

\usepackage{pgfplots}
 \pgfplotsset{compat=newest}
    \pgfplotsset{plot coordinates/math parser=false}
    \pgfplotsset{
    label style={anchor=near ticklabel},
    xlabel style={yshift=0.0em},
    ylabel style={yshift=-0.3em},
    tick label style={font=\footnotesize },
    label style={font=\footnotesize},
    legend style={font=\footnotesize},
    title style={font=\fontsize{7}}}
%\usepackage{xcolor}

\usepackage{mathtools}
\mathtoolsset{showonlyrefs}

\usepackage{placeins}

\usepackage{multirow}
\usepackage{etoolbox}
\usepackage{hhline}

\usepackage{ulem,soul}
\usepackage{balance} 
\usepackage{ctable}

\newcommand\bigzero{\makebox(0,0){\text{\huge$\mathbf{0}$}}}
\newcommand{\ctext}[3][RGB]{%
	\begingroup
	\definecolor{hlcolor}{#1}{#2}\sethlcolor{hlcolor}%
	\hl{#3}%
	\endgroup
}
\newcommand{\old}[1]{\textcolor{gray}{#1}}
\newcommand{\GL}{}
\newcommand{\GLC}{}
\newcommand{\GLS}{}
\newcommand{\fran}{}
\newcommand{\alex}{}
\newcommand{\todo}{}


\newcommand{\E}[1]{{\color{red}#1}}
\newcommand{\EBY}[1]{{\color{red}#1}}

\normalem


==> SRLMP ISIT2021 arxiv/tex_files/prelim.tex <==
\section{Preliminaries}\label{sec:Prelim}



\subsection{Q-ary Symmetric Channel}

Consider a \ac{QSC} with error probability $\proberror$, input alphabet $\inputalphabet$ and output alphabet $\outputalphabet$, with  ${\inputalphabet = \outputalphabet = \{0, \alpha^0, \hdots, \alpha^{q-2}\}}$, where $\alpha$ is a primitive element of $\Fq$. 
Denote by $x \in \inputalphabet$  and $y \in \outputalphabet$ the channel input and channel output, respectively.
The transition probabilities of a \ac{QSC} with error probability $\proberror$ are
\begin{equation}\label{eq:QSC_trans_prob}
P(y|x) =  \begin{cases}
1 - \proberror & \mbox{if } \outputrvreal = \inputrvreal \\
\proberror / (q-1) & \mbox{otherwise}.
\end{cases} 
\end{equation}
The capacity of the \ac{QSC}, in symbols per channel use, is
\begin{equation}\label{eq:capacity_q}
C= 1 + \proberror \log_q \frac{\proberror}{q-1} + (1-\proberror) \log_q (1-\proberror).
\end{equation}


\subsection{Log-Likelihood Vector}
For a given channel output $y$ of a \ac{DMC} with input alphabet $\cX=\Fq$,  we introduce the normalized log-likelihood vector, also referred to as \acl{llv},
	\begin{equation}\label{eq:llvector}
	\bm{L}(y)=\left[ L_0(y), L_1(y), \ldots , L_{\alpha^{q-2}}(y)\right]
	\end{equation}
	whose elements are defined as
	\begin{align}\label{eq:llvector2}
	L_\genfq(y)=& \log \left(P(y|\genfq) \right) \quad \forall u \in \Fq.
	\end{align}
	The \acl{llv}  will be fundamental to the development of a  decoding algorithm for non-binary \ac{LDPC} codes over the \ac{QSC}. In particular, we will focus on  a message passing decoding algorithm where the  exchanged messages are list of symbols  from $\Fq$ of size at most $\Gamma$. In this case, a message sent from a \ac{CN} to a \ac{VN} can be modeled as the observation of the \ac{RV} $X$ after transmission over a $q$-ary input $|\cM_{\Gamma}|$-ary output discrete memoryless extrinsic channel \cite[Fig.~3]{ashikhmin_EXIT}, where $\cM_{\Gamma}$ is the message alphabet. In the decoding algorithm, we will use the 
	\acl{llv} $\bm{L}(y)$ of the communication channel observation and the \aclp{llv} of the \ac{CN} messages $\bm{L}(m), \forall m \in \cM_\Gamma$. While the transition probabilities of the communication channel, which is a \ac{QSC} with error probability $\epsilon$, are given in \eqref{eq:QSC_trans_prob},  the transition probabilities of the extrinsic channel are in general unknown but accurate estimates can be obtained via \ac{DE} analysis, as suggested in \cite{lechner_analysis_2012}.
	
	
	
\subsection{Non-binary LDPC Codes}
Consider next non-binary \ac{LDPC} codes defined by an $m \times n$ sparse parity-check matrix $\bm{H}$ with coefficients in $\Fq$. The parity-check matrix can be represented by a Tanner graph with $n$ \acp{VN} corresponding to codeword symbols and $m$ \acp{CN} corresponding to parity checks.  The edge label associated to the edge connecting  $\vn$ and  $\cn$ is denoted by $h_{\vn,\cn}$, with $h_{\vn,\cn} \in \Fqz$. The sets $\cN(\vn)$ and $\cN(\cn)$ denote the neighbors of \ac{VN} $\vn$ and \ac{CN} $\cn$, respectively. The degree  of a \ac{VN} $\vn$  is the cardinality of the set $\cN(\vn)$. Similarly, the degree of a \ac{CN} $\cn$  is the cardinality of the set $\cN(\cn)$.
The \ac{VN} edge-oriented degree distribution polynomial of an \ac{LDPC} code graph is given by 
$
    \lambda(x)= \sum_{i}\lambda_{i}x^{i-1}
$
where $ \lambda_{i} $ corresponds to the fraction of edges incident to \ac{VN}s with degree $i$.
Similarly, the \ac{CN} edge-oriented degree distribution polynomial is given by
$
\rho \left(x\right) = \sum_{i}\rho_{i}x^{i-1}
$
where $ \rho_{i} $ corresponds to the fraction of edges incident to \ac{CN}s with degree $ i $.
An unstructured irregular \ac{LDPC} code ensemble $\Cirreg$ is the set of all $q$-ary \ac{LDPC} codes with block length $ n $ and degree distributions $ \lambda\left( x\right) $ and $ \rho\left( x\right) $ and  edge labels uniformly chosen in $\Fqz$.



\iffalse
\subsubsection{Protograph Ensembles}
Non-binary protograph-based \ac{LDPC} codes are created from a small Tanner graph called a protograph by a copy-permute-scale procedure \cite{dolecek_non-binary_2014}. The protograph consists of $n_0$ VNs and $m_0$ CNs. Each \ac{VN}/\ac{CN} in a protograph defines a variable/check node type. A protograph can be defined by an $m_0 \times n_0$ base	matrix $\bm{B}= [b_{i,j}]$, where $b_{i,j}$ is the number of edges that connects $\vn_j$ to $\cn_i$. In order to obtain the non-binary parity-check matrix $\bm{H}$, a number of copies of the protograph is generated and their edges are permuted such that connectivity constraints imposed by the base matrix are maintained followed by scaling each edge in the obtained Tanner graph by an element from $\Fqz$. Note that each \ac{VN}/\ac{CN} in a protograph defines a variable/check node type.
\fi


==> SRLMP ISIT2021 arxiv/tex_files/results.tex <==
\section{Numerical Results} \label{sec:results}
\begin{table}[t]
	\centering
	\caption{Decoding thresholds $\epsilon^\star$ of \EBY{the}  $(3,5)$ regular  LDPC code ensemble}
	\begin{tabular}{cccccccc}
		\thickhline  
		\multirow{2}{*}{$q$}&\cite{kurkoski_list}&\ac{SMP}&$\epsilon^\star$& $\epsilon^\star$ &\multirow{2}{*}{$\epsilon^\star_{\text{BP}}$}& \multirow{2}{*}{$\epsilon_{\text{Sh}}$}   \\
		& $\Gamma=1$ &\cite{smp_lazaro} &$\Gamma=1$ &$\Gamma=2$ & & \\
		\hline
		$2$  &  $0.061$ &$ 0.0611$ & $0.0975$  & $  - $        & $ 0.113$ & $ 0.1461$ \\
		
		$4$  & 0.092    &   $ 0.1226$ & $0.1283 $ & $ 0.1632 $    & $ 0.196$ & $0.2480$   \\
		
		$8$  &0.093 &   $0.1335 $ & $0.1430$  &  $ 0.1918 $   & $ 0.254$ & $ 0.3190$ \\
		
		$16$ & 0.094 &   $0.1381 $ &  $0,1627$ & $ 0.2057$     & $ 0.296$ & $  0.3708 $ \\
		
		$32$ &- &  $ 0.1403$  & $0.1906$  & $ 0.2163$     & $ 0.328$ & $0.4086$  \\
		
		$64$ & - & $ 0.1413$   & $0.2153$  & $ 0.2209$     & $ 0.352$ & $0.4369 $  \\
		\thickhline  
	\end{tabular}
	\vspace{-2mm}
	\label{tab:3,5}
\end{table} 


\begin{table}[t]
	\centering
	\caption{Decoding thresholds $\epsilon^\star$ of  \EBY{the}  $(3,4)$  regular LDPC code ensemble}
	\begin{tabular}{ccccccc}
		\thickhline  
		\multirow{2}{*}{$q$}&\cite{kurkoski_list}&\ac{SMP}&$\epsilon^\star$& $\epsilon^\star$ &\multirow{2}{*}{$\epsilon^\star_{\text{BP}}$}& \multirow{2}{*}{$\epsilon_{\text{Sh}}$}   \\
		& $\Gamma=2$ &\cite{smp_lazaro} &$\Gamma=1$ &$\Gamma=2$ & & \\
		\hline
		$2$  & -     & $ 0.1069$ & $0.1439$   &$ - $    & $0.167$    &  $ 0.2145$ \\
		$4$  & 0.222 & $0.1724$  & $0.1842$   &$0.2390$ & $0.2804$   &$0.3546 $  \\
		$8$  & 0.269 & $0.1867$  & $0.2096$   &$ 0.2790$& $ 0.355$   & $0.4480 $   \\
		$16$ & 0.287 & $0.1930$  & $0.2481$   &$0.2977$ & $0.4076$   &$  0.5120$  \\
		$32$ & -     & $0.1960$  & $0.2893$   &$0.3110$ &$0.4446 $   &$ 0.5570$ \\
		$64$ & -     & $0.1974 $ & $0.3128$   &$0.3175$ &$ 0.4757$   &$ 0.5894$ \\
		\thickhline  
	\end{tabular}
	\vspace{-2mm}
	\label{tab:3,4}
\end{table} 

We investigate the asymptotic performance of \ac{SRLMP} with maximum list size $1$ and $2$ obtained by \ac{DE}. Tables \ref{tab:3,5} and \ref{tab:3,4} show the iterative decoding thresholds of \ac{SRLMP} for $(3,4)$ and $(3,5)$ regular ensembles and various values of $q$. For the sake of comparison, we provide the belief propagation thresholds $\epsilon^\star_{\text{BP}}$, the Shannon limit $\epsilon_{\text{Sh}}$ and the thresholds of the  \ac{SMP} decoder \cite{smp_lazaro}, which is similar to the \ac{SRLMP} with $\Gamma=1$ (excluding the empty set). By comparing the  thresholds for $\Gamma=1$ with the  \ac{SMP} ones, we see that significant gains are obtained if empty sets are allowed in the decoding algorithm. Increasing $\Gamma$  improves the threshold but this comes at the cost of an increasing complexity. We believe that increasing $\Gamma$ further  will significantly increase the  decoding complexity and  will not achieve significant gains compared to the case of $\Gamma=2$.
Note that the \ac{SRLMP} outperforms the decoding algorithm in \cite{kurkoski_list} for the same maximum list size.



 Since the \ac{CN} update rule of both decoders is the same, the gain is probably due to the \ac{VN} update rule which is more complex for the case of the \ac{SRLMP} decoder. In fact, the \acp{VN} in \cite{kurkoski_list} compute the sum of binary vectors, whereas, here the incoming messages are converted to \aclp{llv} before summation.
To check the finite-length performance under \ac{SRLMP}, we consider the performance of a regular  $(3,5)$ code  where we set the maximum number of iterations $\ell_\tmax= 50$. The code has a block length $n=60000$  and its Tanner graph is obtained via the \ac{PEG} algorithm \cite{Hu_peg}. Finite-length simulation results for $\Gamma=1$ and $\Gamma=2$ are shown in Fig.\ref{fig:results_sim_3_5q4} in terms of \ac{SER} versus the \ac{QSC} error probability $\proberror$. We keep $\Delta^{(\ell)}$ constant over the iterations and  use $\Delta^{(\ell)}= 1$ for $\Gamma = 1$  and $ \Delta^{(\ell)}=1.25 $ for $\Gamma=2$.
  As a reference, we  provide the simulation results  under the \ac{SMP} decoder \cite{smp_lazaro} and under the decoding algorithm in   \cite{kurkoski_list} for $\Gamma=1$.


 




\begin{figure}[t]
	\centering
	\footnotesize
	\includegraphics{figures/fig_SRLMP}
	\caption{\ac{SER} versus channel error probability $\proberror$ for $4$-ary regular $(3,5)$ \ac{LDPC} code with $n=60000$.}
	\label{fig:results_sim_3_5q4}
	\vspace{-2mm}
\end{figure}




==> tex_files/notation.tex <==
\newtheorem{remark}{Remark}



\newcommand{\dv}{\mathsf{d_{v}}}
\newcommand{\dc}{\mathsf{d_{c}}}
\newcommand{\dvj}{\mathsf{d_{v_{j}}}}
\newcommand{\dci}{\mathsf{d_{c_{i}}}}
\newcommand{\dvmax}{\mathsf{d_{v}^{\text{max}}}}
\newcommand{\dcmax}{\mathsf{d_{c}^{\text{max}}}}

\newcommand{\inputalphabet}{\mathcal{X}}
\newcommand{\inputrv}{X}
\newcommand{\inputrvreal}{x}
\newcommand{\outputalphabet}{\mathcal{Y}} 
\newcommand{\outputrv}{Y}
\newcommand{\outputrvreal}{y}

\newcommand{\messagealphabet}{\mathcal{M}}

\newcommand{\proberror}{\epsilon}
\newcommand{\proberasure}{\gamma}
\newcommand{\ns}{{\eta}}

\newcommand{\normterm}{\delta}
	
\newcommand{\Rc}{R}

\newcommand{\Cirreg}{\mathscr{C}_{q}^{\lambda,\rho}}
\newcommand{\ensC}[3]{\mathscr C_{ #1, #2}^{#3}}
\newcommand{\ensSC}[3]{\bm{B}_{ #1, #2}^{#3}}
\newcommand{\vn}{\mathtt{v}}%variable node

\newcommand{\cn}{\mathtt{c}}%check node

\newcommand{\cm}{r}%channel message


\newcommand{\cN}{\mathcal{N}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cI}{\mathcal{I}}


\newcommand{\vcm}[2]{p_{#1}^{(#2)}}%pr  of var to check node message
\newcommand{\cvm}[2]{s_{#1}^{(#2)}}
\newcommand{\cvmvec}[1]{\bm{s}^{(#1)}}
\newcommand{\vcmvec}[1]{\bm{p}^{(#1)}}
\newcommand{\vcmvecFP}{\bm{p}^{\star}}
\newcommand{\cvmvecFP}{\bm{s}^{\star}}


\newcommand{\vcmirreg}[2]{\bar{p}_{#1}^{(#2)}}%pr  of var to check node message
\newcommand{\cvmirreg}[2]{\bar{s}_{#1}^{(#2)}}

\newcommand{\vapp}[1]{P_{\tapp}^{(#1)}} %decision variable node
\newcommand{\vcmlong}[2]{P_{\outputrv|\inputrv}^{(#2)}(#1|0) }%pr  of var to check node message
\newcommand{\cvmlong}[2]{P_{S|\inputrv}^{(#2)}(#1|0) }%pr  of var to check node message
\newcommand{\vcmFP}[1]{p_{#1}^{\star}}
\newcommand{\cvmFP}[1]{s_{#1}^{\star}}


\newcommand{\vect}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\neigh}[1]{\mathcal{N} ( #1) }



\newcommand{\mes}[3]{m_{ #1 \rightarrow #2 }^{(#3)}}
\newcommand{\Mes}[3]{M_{ #1 \rightarrow #2 }^{(#3)}}

\newcommand{\mesch}[1]{m_{ #1 }}

\newcommand{\minr}{m_{ \text{in}}}
\newcommand{\minrv}[1]{M^{(#1)}_{ \text{in}}}

\newcommand{\vecgen}{u}

\newcommand{\comp}{{\Psi}}

\newcommand{\Fq}{\mathbb{F}_q}
\newcommand{\Fqz}{\mathbb{F}_q \setminus \{0\}}
\newcommand{\Fqa}{\mathbb{F}_q \setminus \{a\}}

\renewcommand{\argmax}[1]{\underset{#1}{\mathrm{arg \, max}}\,}

\newcommand{\mesvec}[2]{\bm{z}_{#1 \rightarrow #2}}

\ifdef{\l}
{\renewcommand{\l}[1]{L_{ #1}} }
{\newcommand{\l}[1]{L_{ #1}}}

\newcommand{\lv}{\bm{L}}

\newcommand{\lin}[1]{\sigma^{(#1)}}
\newcommand{\linv}[1]{\bm{\sigma}^{(#1)}}

\newcommand{\linapp}[1]{l^{(#1)}}
\newcommand{\linappv}[1]{\bm{l}^{(#1)}}

\newcommand{\papp}[1]{P_{\text{app}}^{(#1)}}

\newcommand{\genfq}{u}



\newcommand{\linvi}[3]{\bm{l}_{ #1 \rightarrow #2}^{(#3)} }
\newcommand{\lini}[3]{l_{ #1 \rightarrow #2}^{(#3)} }

\newcommand{\lch}[1]{l_{\text{ch}, #1}}
\newcommand{\lchv}{\bm{l}_{\text{ch}}}

\newcommand{\F}[1]{F_{#1}}
\newcommand{\f}[1]{f_{#1}}
\newcommand{\tF}[1]{\tilde{F}_{#1}}
\newcommand{\tf}[1]{\tilde{f}_{#1}}

\newcommand{\Fv}{\bm{F}}
\newcommand{\fv}{\bm{f}}
\newcommand{\tFv}{\bm{\tilde{F}}}
\newcommand{\tfv}{\bm{\tilde{f}}}

\newcommand{\fve}{\bm{f}}
\newcommand{\Fe}[1]{F_{#1}}
\newcommand{\fe}[1]{f_{#1}}
\newcommand{\tFe}[1]{\tilde{F}_{#1}}
\newcommand{\tfe}[1]{\tilde{f}_{#1}}
\newcommand{\Fve}{\bm{F}}
\newcommand{\tFve}{\bm{\tilde{F}}}
\newcommand{\tfve}{\bm{\tilde{f}}}


\newcommand{\fvl}{\bm{f}}
\newcommand{\Fl}[1]{F_{\{#1\}}}
\newcommand{\fl}[1]{f_{\{#1\}}}
\newcommand{\Flp}[2]{F_{\{#1\},#2}} %proto
\newcommand{\flp}[2]{f_{\{#1\},#2}}
\newcommand{\tflp}[2]{\tilde{f}_{\{#1\},#2}}
\newcommand{\tFl}[1]{\tilde{F}_{\{#1\}}}
\newcommand{\tfl}[1]{\tilde{f}_{\{#1\}}}
\newcommand{\Fvl}{\bm{F}}
\newcommand{\tFvl}{\bm{\tilde{F}}}
\newcommand{\tfvl}{\bm{\tilde{f}}}



\newcommand{\Dch}{D_{\text{ch}}}
\newcommand{\Dex}{D_{\text{ex}}}

\newcommand{\I}{\mathbb{I}}
\newcommand{\argI}{\mathcal B}

\renewcommand{\a}{a}
\renewcommand{\b}{y}
\renewcommand{\u}{u}

\newcommand{\nbit}{l}
\newcommand{\hw}{\mathrm d_{\mathrm{H}}}

\newcommand{\cellfreq}{z}

\newcommand{\agg}{L_{\mathsf{ex}}}
\newcommand{\aggc}[2]{L^{(#2)}_{\mathsf{ex},#1}}
\newcommand{\aggv}[1] {\bm{L}^{(#1)}_{\mathsf{ex}}}
\newcommand{\lmaxim}[1]{\mathcal{L^{(#1)}_{\mathsf{ex}}}}

\newcommand{\aggappvl}[1]{{\bm{L}^{(#1)}_{\mathsf{app}}}} %app l-th iteration
\newcommand{\aggappl}[2]{{L^{(#2)}_{\mathsf{app},#1}}}
\newcommand{\lmaximapp}[1]{\mathcal{L^{(#1)}_{\mathsf{app}}}}

\newcommand{\Mcdf}{P}
\newcommand{\Mpdf}{\rho}

\newcommand{\Xa}{A}
\newcommand{\xa}{a}
\newcommand{\Ya}{B}
\newcommand{\ya}{b}

\newcommand{\binv}[1]{\bm{#1}_{\mathrm{b}}}
\newcommand{\mapbin}[1]{{_b}\left(#1\right) }

\ifdef{\H}
{\renewcommand{\H}{\mathsf{U}}}
{\newcommand{\H}{\mathsf{U}}}

\ifdef{\D}
{\renewcommand{\D}{\mathsf{D}}}
{\newcommand{\D}{\mathsf{D}}}

\newcommand{\W}{\mathsf{W}}

\newcommand{\nmax}[1] { \underset{#1}{\#\mathrm{max} }} %
\newcommand{\nel}[1]{{\mu}_{#1} } %
\newcommand{\nmaxr}{\kappa}
\newcommand{\nmaxrmax}{\kappa_{\mathrm{max}}}


\newcommand{\accvote}[1]{{t_{#1}}}
	
\newcommand{\az}{\accvote{0}}
\newcommand{\ao}{\accvote{1}}


\newcommand{\fmax}{f_{\text{max}}}


\newcommand{\tapp}{\text{app}}
\newcommand{\tmax}{\text{max}}
\newcommand{\tch}{\text{ch}}

\newcommand{\lmp}{LMP }
\newcommand{\e}{\mathcal{E}} % erasure 

==> tex_files/packages.tex <==
\usepackage{amsmath,amsthm,amssymb,graphicx,cite,bm}
\usepackage{epsfig,amsfonts}
\usepackage{graphicx}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\usepackage[nolist]{acronym}
\usepackage{psfrag}
\usepackage{perso}
\usepackage{makecell}
\usepackage{enumitem}
\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother
%
%\bibliographystyle{IEEEtran}
%\setlength{\arraycolsep}{0.07 cm}
%
%\IEEEoverridecommandlockouts

\usepackage{pgfplots}
 \pgfplotsset{compat=newest}
    \pgfplotsset{plot coordinates/math parser=false}
    \pgfplotsset{
    label style={anchor=near ticklabel},
    xlabel style={yshift=0.0em},
    ylabel style={yshift=-0.3em},
    tick label style={font=\footnotesize },
    label style={font=\footnotesize},
    legend style={font=\footnotesize},
    title style={font=\fontsize{7}}}
%\usepackage{xcolor}

\usepackage{mathtools}
\mathtoolsset{showonlyrefs}

\usepackage{placeins}

\usepackage{multirow}
\usepackage{etoolbox}
\usepackage{hhline}

\usepackage{ulem,soul}
\usepackage{balance} 
\usepackage{ctable}

\newcommand\bigzero{\makebox(0,0){\text{\huge$\mathbf{0}$}}}
\newcommand{\ctext}[3][RGB]{%
	\begingroup
	\definecolor{hlcolor}{#1}{#2}\sethlcolor{hlcolor}%
	\hl{#3}%
	\endgroup
}
\newcommand{\old}[1]{\textcolor{gray}{#1}}
\newcommand{\GL}{}
\newcommand{\GLC}{}
\newcommand{\GLS}{}
\newcommand{\fran}{}
\newcommand{\alex}{}
\newcommand{\todo}{}


\newcommand{\E}[1]{{\color{red}#1}}
\newcommand{\EBY}[1]{{\color{red}#1}}

\normalem

